SO(3) attitude controllers and the alignment of robots with non-constant 3D vector fields

This technical note aims to introduce geometric controllers to roboticists for aligning \emph{3D robots} with non-constant 3D vector fields. This alignment entails the control of the robot's 3D attitude. We derive with excessive detail all the calculations needed for the analysis and implementation of the controllers.

==> Makefile <==
all: main.pdf

clean:
	$(RM) *~ *.pdf *.dvi *.log *.aux *.bbl *.blg *.toc *.lol *.loa *.lox \
		*.lot *.out *.lg *.tmp *.xref *.lof .*.swp *.synctex.gz

main.pdf: main.tex
	pdflatex main
	bibtex main
	pdflatex main
	pdflatex main

